Okay, Let's Do This! Modeling Event Coreference with Generated Rationales and Knowledge Distillation

In NLP, Event Coreference Resolution (ECR) is the task of connecting event clusters that refer to the same underlying real-life event, usually via neural systems. In this work, we investigate using abductive free-text rationales (FTRs) generated by modern autoregressive LLMs as distant supervision of smaller student models for cross-document coreference (CDCR) of events. We implement novel rationale-oriented event clustering and knowledge distillation methods for event coreference scoring that leverage enriched information from the FTRs for improved CDCR without additional annotation or expensive document clustering. Our model using coreference specific knowledge distillation achieves SOTA B3 F1 on the ECB+ and GVC corpora and we establish a new baseline on the AIDA Phase 1 corpus. Our code can be found at https://github.com/csu-signal/llama_cdcr

==> reviews.tex <==
Checklist:
1. We will make the dashed blue line bolder so it is easier to see and redirect through the Student (Longformer) box to make clear that the rationale representation is encoded by the Student in this step.

2. We’ll add this description to the Fig. 1 caption about the representative rationales (R). We’ll also make the a/b/c in each colored cluster distinct letters (d/e/f, g/h/i, etc.) to make clear that these denote distinct mentions. 
--additional text descriptions about mentions and R with colors are added to caption. 

3. Typo in Task Instructions in figure 2, Identity -> Identify? DONE!
Thank you for catching that.  We’ll fix it.



mtjv:


Summary Of Strengths:
The idea is novel and interesting. The proposed method only requires the generated rationales during the training time not the inference time, which increases the usability of the model.
Summary Of Weaknesses:
Although authors evaluated the quality of generated rationales, it would be helpful to have some analysis on how the quality affects the resolver's performance.
The model assumes that the event mentions are provided. It would be more useful if the model is end-to-end.
Comments, Suggestions And Typos:
In section 3.3, the rationale representation is generated by the student model, while it is unclear in Figure 1.
In Figure 1, it better to have some descriptions about the "a", "b","c" of color red, blue, green in the box of ROEC. It is a bit unclear to me.
Have you considered to use proposed method on within-doc coreference resolution task?
Typo in Task Instructions in figure 2, Identity -> Identify?
Soundness: 4 = Strong: This study provides sufficient support for all of its claims/arguments. Some extra experiments could be nice, but not essential.
Overall Assessment: 4 = This paper represents solid work, and is of significant interest for the (broad or narrow) sub-communities that might build on it.


Confidence: 4 = Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.
Reproducibility: 4 = They could mostly reproduce the results, but there may be some variation because of sample variance or minor variations in their interpretation of the protocol or method.
Datasets: 1 = No usable datasets submitted.
Software: 3 = Potentially useful: Someone might find the new software useful for their work.

Our response:
Thank you for your thoughtful review and recognizing the novelty and utility of the presented work. In our response, numbered citations reference the list provided under the Official Comment to the original submission.

> Although authors evaluated the quality of generated rationales, it would be helpful to have some analysis on how the quality affects the resolver's performance.
Human evaluation of the rationales is relatively time consuming. Performing evaluation over all rationales (~41K for ECB+ at 1 rationale per mention pair), or even a representative sample, is intractable without large-scale crowdsourcing via a platform like MTurk, which was unfortunately precluded for budget reasons. This can be a topic of future work, such as using a critic model to select which rationales should be included in knowledge distillation (Section 7).

> The model assumes that the event mentions are provided. It would be more useful if the model is end-to-end.
We took this approach in order to make a direct comparison with previous work, who also evaluate their coreference resolution models assuming access to gold coreference mentions [1–12] on datasets like ECB+. Works such as Bugert et al. [9] suggest that most event CDCR corpora (e.g., ECB+) under-annotate event mentions. As such, end-to-end CDCR systems that include event detection are prone to detecting unannotated mentions that are then incorrectly merged into large clusters that drastically reduce performance of the resolution component. Therefore, apart from Cattan et al. [5] that includes such a step, many previous works have avoided it in order to demonstrate their resolution systems. As such, we follow standard practice [9] in presenting our results, but our modular pipeline could easily be hooked up to a mention detector such as Cattan et al’s [5] for a fully end-to-end system.

> In section 3.3, the rationale representation is generated by the student model, while it is unclear in Figure 1.
There is a dashed blue line from the rationale on the right to the “Event Mention Representation” box on the left, that indicates this.  All green boxes in Fig. 1 indicate the student model or its outputs and all blue boxes indicate the teacher model or its outputs. Nonetheless, we see how this could be unclear. We will make the dashed blue line bolder so it is easier to see and redirect through the Student (Longformer) box to make clear that the rationale representation is encoded by the Student in this step.

> In Figure 1, it better to have some descriptions about the "a", "b","c" of color red, blue, green in the box of ROEC. It is a bit unclear to me.
“a”, “b”, “c” represent event mentions, and the colors represent an event cluster (such that all the blue circles cluster together). “R” represents a set of rationales that justify the linking of different mentions in a single cluster. We’ll add this description to the Fig. 1 caption. We’ll also make the a/b/c in each colored cluster distinct letters (d/e/f, g/h/i, etc.) to make clear that these denote distinct mentions.

> Have you considered to use proposed method on within-doc coreference resolution task?
Standard CDCR corpora like ECB+ include both within and cross-document coreference link annotations, and most recent event CDCR systems [2, 4, 5–8, 10, 11] report system performance on the full gold annotations (including within-doc links) for a more exhaustive evaluation (as do we). While [2, 12] report within-doc performance on ECB+ separately, cutting out cross-document links renders most mentions in ECB+ as singletons, since most coreference links in ECB+ cross documents (~1.24 average cluster size for within-doc clusters vs. ~14 for cross-doc). This results in an artificial performance boost in B3 and CEAFe metrics (thereby boosting CoNLL F1). MUC remains unaffected but [13] suggests that MUC is the least discriminative metric and hence, less reflective of final cluster purity. As such, we provide results on the full CDCR corpora like most previous work mentioned above. It would be simple for us to separate the within-doc links alone and evaluate on those, but as the focus of this paper is to demonstrate a novel CDCR technique, we devote our space to evaluating in line with existing standard CDCR practice.

> Typo in Task Instructions in figure 2, Identity -> Identify?
Thank you for catching that.  We’ll fix it.


QNwz:

Summary Of Strengths:
The approach is intuitive and the technical aspects of the paper are easy to follow. The three core contributions are explained thoroughly
New SOTA on B3 F1 for three corpora is achieved. The authors also provide zero-shot baselines with GPT 3.5 and LLaMA-2-chat to show that a strong LLM alone is not sufficient.
Ablation results are included and emphasize the strength of the model
A new baseline on the AIDA Phase 1 corpus is provided
Summary Of Weaknesses:
Only 1 evaluation metric of B3. While results are SOTA for this one metric, perhaps for other metrics we do not see the same signal. Ahmed et al 2023 seemed to have used other common ECE metrics.
Comments, Suggestions And Typos:
See above. With newer models coming out, I am curious how these results will hold with models like Mistral-7B-Chat, GPT-4, etc. I am also curious about how many samples were thrown out due to safety filters on LLMs?
Soundness: 3.5
Overall Assessment: 3.5
Confidence: 3 =  Pretty sure, but there's a chance I missed something. Although I have a good feel for this area in general, I did not carefully check the paper's details, e.g., the math or experimental design.
Reproducibility: 5 = They could easily reproduce the results.
Datasets: 4 = Useful: I would recommend the new datasets to other researchers or developers for their ongoing work.
Software: 4 = Useful: I would recommend the new software to other researchers or developers for their ongoing work.

Our response:
Thank you for your review recognizing our core contributions, the intuitiveness of our approach, and the utility of our data and pipeline. In our response, numbered citations reference the list provided under the Official Comment to the original submission.

> Only 1 evaluation metric of B3. While results are SOTA for this one metric, perhaps for other metrics we do not see the same signal. Ahmed et al 2023 seemed to have used other common ECE metrics.

We do provide other coreference metrics in Appendix D for future reproduction and comparison. On the metrics where we don’t achieve SOTA, we remain extremely competitive (see MUC F1, CEAFe F1, and CoNLL-F1 on both ECB+ and GVC in Tables 5–7). Our reasons for focusing on B3 in the main body of the paper follow: Ahmed et al. [8] primarily present CoNLL-F1 score, and compare to Held et al. [7]. They beat Held et al. using their “oracle assumption” for candidate generation while pruning the long tail of non-coreferring pairs. However, since the oracle assumption assumes access to the test set for candidate generation, we cannot use it and maintain a direct comparison on the same test samples. Therefore we use Ahmed’s non-oracle assumption for preprocessing. Using the non-oracle assumption, Ahmed et al. do not beat Held et al.’s performance, meaning that when using this preprocessing method, Held et al. remains the pertinent SOTA model to compare to.  Since Held et al. make their primary comparisons on the B3 metric, so do we.

> With newer models coming out, I am curious how these results will hold with models like Mistral-7B-Chat, GPT-4, etc.

With GPT-4 being a closed model, it is of limited utility for our knowledge distillation process since we cannot access the weights. Budget constraints precluded using GPT-4 for zero-shot coreference since we’d have to pay OpenAI for a large number of requests to the service. The Mistral model is quite new and not set up on our servers at time of writing, but our pipeline allows for another open-weight model to be dropped in in place of LLaMA and our code will be made public upon publication, allowing future research on precisely this type of interesting question.

> I am also curious about how many samples were thrown out due to safety filters on LLMs?

This is mentioned in Limitations. 167 AIDA and 70 GVC samples (pairs) were thrown out because LLaMA 2 would not generate an answer during zero-shot coreference.







APKL:


Summary Of Strengths:
The proposed method for incorporating rationales into the modeling of coreferent event pairs and the corresponding ablation study.
Summary Of Weaknesses:
The lack of strong baselines and sota models for coreference resolution -- the field has advanced way beyond simple mention-pair encodings using a longformer backbone.
Comments, Suggestions And Typos:
How does your proposed approach compare to existing state of the art conference resolvers?
How much of an impact do the quality of the generated rationals has on the final performance?
Soundness: 3 = Acceptable: This study provides sufficient support for its major claims/arguments. Some minor points may need extra support or details.
Overall Assessment: 2.5
Confidence: 4 = Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.
Best Paper: No
Ethical Concerns:
None
Needs Ethics Review: No
Reproducibility: 4 = They could mostly reproduce the results, but there may be some variation because of sample variance or minor variations in their interpretation of the protocol or method.
Datasets: 3 = Potentially useful: Someone might find the new datasets useful for their work.
Software: 2 = Documentary: The new software will be useful to study or replicate the reported research, although for other purposes it may have limited interest or limited usability. (Still a positive rating)

Our response:
Thank you for your review and acknowledging the strength of our presented method and experiments. In our response, numbered citations reference the list provided under the Official Comment to the original submission.

It is important to note that our work focuses on the specific problem of cross-document event coreference resolution (event CDCR; mentioned in Abstract, Section 1, Section 2, etc.) and that there are some substantial technical differences between CDCR and within-document coreference resolution (WDCR) that determine the models we compare to. 

> The lack of strong baselines and sota models for coreference resolution -- the field has advanced way beyond simple mention-pair encodings using a longformer backbone.

To the best of our knowledge, most recent SOTA works [6–8, 14] on event CDCR still work within a mention-pair encoding framework with innovations mostly centered around feature-enhancement techniques like longer-context [6], discourse-coherence/structure theory [7, 14] or lemma-based pruning [8]. We compare our results with all these except Chen et al.  [14] which was only published a week before the deadline. While more sophisticated mention-ranking or even entity-level modeling has been explored previously [17–20], such systems only resolve within-doc coreference. CDCR systems, on the other hand, cannot directly use the innate coherence within a document for such ranking architectures since mentions of the same event overwhelmingly occur in different documents in common CDCR corpora like ECB+. The intractability of finding candidates across documents (~n^2 complexity even after document clustering) means pairwise scoring after the document clustering/pruning step remains a simple yet effective, and therefore standard, method for this task. While a simple pairwise scoring could technically violate innate transitivity of coreference relations, during inference we also use an affinity-based clustering step (different from ROEC, and following [4-12, 15]) after mention-pair scoring to tackle such violations (see Section 4). Other very recent event-CDCR works like [15, 16] also use the mention-pair framework while using generative AI for feature enhancement or event annotations. We do not compare to [15] since they only report results without singletons and [16] does not directly resolve event coreference as they focus on event-type classification. 

Please see our response to Reviewer mtjv regarding the question of how our system handles within-document coreference links (where we follow standard practice in CDCR).   

> How does your proposed approach compare to existing state of the art conference resolvers?
We compare to Cattan et al. (2021), Caciularu et al. (2021), Held et al. (2021), and Ahmed et al. (2023) [5–8]. These are the state of the art resolvers in CDCR (not in strictly within-doc coreference as noted above). For example, Chen et al. (published at EMNLP 2023 one week before the NAACL deadline) [14] presents comparisons to [5–7] (albeit only on ECB+ where we test on 3 datasets). Therefore we can confidently assert that our approach beats or remains competitive with SOTA CDCR on the many different coreference metrics, on multiple datasets.

> How much of an impact do the quality of the generated rationals has on the final performance?
This remains the topic of future work due to the labor (and therefore budget) requirements for a human quality evaluation over rationales generated for an ECR corpus or representative sample thereof (see response to reviewer mtjv).  Now that we have demonstrated the utility of rationales for coreference in general, the question of the effect of rationale quality is ripe for future work.

